Relatively Complete Verification of Probabilistic Programs

We study a syntax for specifying quantitative "assertions" - functions mapping program states to numbers - for probabilistic program verification. We prove that our syntax is expressive in the following sense: Given any probabilistic program $C$, if a function $f$ is expressible in our syntax, then the function mapping each initial state $\sigma$ to the expected value of $f$ evaluated in the final states reached after termination of $C$ on $\sigma$ (also called the weakest preexpectation $\textit{wp} [C](f)$) is also expressible in our syntax. As a consequence, we obtain a relatively complete verification system for reasoning about expected values and probabilities in the sense of Cook: Apart from proving a single inequality between two functions given by syntactic expressions in our language, given $f$, $g$, and $C$, we can check whether $g \preceq \textit{wp} [C] (f)$.

==> body.tex <==
% !TEX root = ./main.tex

\input{introduction}

\input{extensional}

\input{towards}

\input{syntax}

\input{semantics}

\input{proof_straight_line}

\input{proof_outline}


%\input{multiplication}

\input{first_order_arithmetic}
% Bibliography

\input{normalforms}

\input{sums_prod_goedel}

%\input{pgcl_wp}

\input{expressiveness}

\input{applications}

\input{conclusion}

\bibliography{literature}


==> keywords.tex <==
\lstset{
    language=C,%
    %numbers=left,%
    %stepnumber=4,%
    alsoletter={<,>,:=,[,],.},
    morekeywords={
            skip,%
            new,%
            free,%
            call,%
            var,%
            procedure,%
            uniform,%
            [0.5],%
    },%
    basicstyle=\footnotesize\ttfamily,%
    keywordstyle=\bfseries,%
    commentstyle=\itshape,%
}%


==> multiplication.tex <==
\section{Expressing Products of Syntactic Expectations}
\label{sec:product_of_exp}

\cmcommentinline{I really consider this low priority}
%
\kbcommentinline{It's not. I need this.}
In this section, we address the problem of expressing the product of syntactic expectations. Syntactically, we do not allow for  the multiplication $\FF_1 \cdot \FF_2$ of two \emph{arbitrary} syntactic expectations $\FF_1$ and $\FF_2$. For instance,
%
\[
   \big( \Sup \VV_1 \colon \VV_1 \big) \cdot  \big( \Inf  \VV_2 \colon \VV_2 \big) \not\in \SyntE~.
\]
%
Using the Dedekind normal form, we show, however, that such arbitrary products are expressible in $\SyntE$, i.e.\
%
\begin{align*}
\text{for every $\FF_1, \FF_2 \in \SyntE$, there is an $\FF \in \SyntE$ such that} \quad
\forall \sigma \forall \interpret \colon
\sem{\FF_1}{\sigma}{\interpret} \cdot \sem{\FF_2}{\sigma}{\interpret}  \eeq 
\sem{\FF}{\sigma}{\interpret} ~.
\end{align*}
%
First, we employ an auxiliary result:
%
\begin{lemma}
	\label{lem:aux_products_of_exp}
	Let $\FF_1, \FF_2 \in \SyntE$ be syntactic expectations of the form
	%
	\begin{align*}
	  \FF_1 \eeq \Quant_1 \VV_1 \ldots \Quant_i \VV_i \colon \iverson{\BB_1} 
	  %
	  \quad  \text{and} \quad 
	  \FF_2  \eeq  \Quant'_1 \VV'_1 \ldots \Quant'_j \VV'_j \colon \iverson{\BB_2}
	\end{align*}
	%
	such that $\FF_1$ and $\FF_2$ do not share any (bound or free) logical variable.
	%
	Furthermore, let 
	%
	\[
	   \FF  \eeq
	    \Quant_1 \VV_1 \ldots \Quant_i \VV_i \colon 
	    \Quant'_1 \VV'_1 \ldots \Quant'_j \VV'_j \colon 
	     \iverson{\BB_1} \cdot \iverson{\BB_2}~.
	\]
	%
	For all states $\sigma$ and all interpretations $\interpret$, we have
	%
	\[
	  \sem{\FF_1}{\sigma}{\interpret} \cdot \sem{\FF_2}{\sigma}{\interpret}  \eeq 
	  \sem{\FF}{\sigma}{\interpret}
	\]
\end{lemma}
%
\begin{proof}
	By induction on $i$ and Lemma~\ref{thm:prenex:aux}. See Appendix~\ref{proof:aux_products_of_exp}.
	%
\end{proof}
%
%
Observe that Lemma~\ref{lem:aux_products_of_exp} applies to expectations in Dedekind normal form:
%
\begin{corollary}
	\label{cor:prod_of_dedekind}
	Let 
	%
	\begin{align*}
		\dexp{\FF_1} \eeq \Quant_1 \VV_1 \ldots \Quant_i \VV_i \colon \iverson{\BB_1} 
		%
		\quad \text{and} \quad
		%
		\dexp{\FF_2} & \eeq  \Quant'_1 \VV'_1 \ldots \Quant'_j \VV'_j \colon \iverson{\BB_2}~,
	\end{align*}
	%
	be expectations in Dedekind normal form that do not share any (bound or free) logical variables with cut variables $\VVcutnum{1}$ and $\VVcutnum{2}$, respectively. Furthermore, let 
	%
		\[
		\FF  \eeq
		\Quant_1 \VV_1 \ldots \Quant_i \VV_i \colon 
		\Quant'_1 \VV'_1 \ldots \Quant'_j \VV'_j \colon 
		\iverson{\BB_1} \cdot \iverson{\BB_2}~.
		\]
	%
	For all states $\sigma$ and all interpretations $\interpret$, we have
	%
	\begin{enumerate}
		\item $\sem{\FF}{\sigma}{\interpret} \in \{ 0,1\}$, and
		%
		\item 
		%
		\[
		   \sem{\FF}{\sigma}{\interpret} \eeq 1 
		   \qquad \text{iff} \qquad
		   \interpret(\VVcutnum{1}) \in \dcut{\sem{\FF_1}{\sigma}{\interpret}}
		   ~\text{and}~
		   \interpret(\VVcutnum{2}) \in \dcut{\sem{\FF_2}{\sigma}{\interpret}}~.
		\]
	\end{enumerate}
	
\end{corollary}
%
%
\begin{proof}
	This is an immediate consequence of Theorem~\ref{thm:dedekind_nf}
	and Lemma~\ref{lem:aux_products_of_exp}.
\end{proof}
%
We denote the$\FF$ from above by $\dexp{\FF_1} \cdot \dexp{\FF_2}$ .
%
Next, we employ the well-known fact that for all $A,B \subseteq \PosRats$ it holds that
%
\[
   \sup A \cdot \sup B \eeq \sup \setcomp{\RR_1 \cdot \RR_2}{\RR_1 \in A ~\text{and}~ \RR_2 \in B}~.
\]
%
Hence, the product of $a \cdot b$ of $a, b \in \PosRealsInf$ can be expressed as
%
\begin{align}
\label{eqn:product_by_dedeking_cut}
   a\cdot b \eeq \sup \dcut{a} \cdot \sup \dcut{b}
   \eeq \sup \setcomp{\RR_1 \cdot \RR_2}{\RR_1 \in \dcut{a} ~\text{and} \RR_2 \in \dcut{b}}~.
\end{align}
%
Note that this characterization complies with $0 \cdot \infty = 0$ since
%
\[
   0\cdot \infty \eeq \sup \emptyset \cdot \sup \PosRats
   \eeq \sup \setcomp{\RR_1 \cdot \RR_2}{\RR_1 \in \emptyset ~\text{and} \RR_2 \in \PosRats} \eeq \sup \emptyset \eeq 0~.
\]
%
Hence, we define:
%
\begin{definition}
	\label{def:product_of_exp}
	Let $\FF_1, \FF_2 \in \SyntE$ be expectations that do not share any (bound or free) logical variables, 
	and let
	%
	\begin{align*}
	\dexp{\FF_1} \eeq \Quant_1 \VV_1 \ldots \Quant_i \VV_i \colon \iverson{\BB_1} 
	%
	\quad \text{and} \quad
	%
	\dexp{\FF_2} & \eeq  \Quant'_1 \VV'_1 \ldots \Quant'_j \VV'_j \colon \iverson{\BB_2}~,
	\end{align*}
	%
	with cut variables $\VVcutnum{1}$ and $\VVcutnum{2}$, respectively. We define the \emph{product} $\FF_1 \cdot \FF_2$ of $\FF_1$ and $\FF_2$ by
	%
	\[
	   \FF_1 \cdot \FF_2 \eeq
	   \Sup \VVcutnum{1} \colon \Sup \VVcutnum{2} \colon
	   \VVcutnum{1} \cdot \VVcutnum{2} \cdot \dexp{\FF_1} \cdot \dexp{\FF_2}~.
	\]
\end{definition}
%
%
\begin{theorem}
	For every expectations $\FF_1, \FF_2 \in \SyntE$ that do not share any (bound or free)
	logical variables, we have for every state $\sigma$ and every interpretation $\interpret$,
	%
	\[
	   \sem{\FF_1 \cdot \FF_2}{\sigma}{\interpret}
	   \eeq \sem{\FF_1}{\sigma}{\interpret} \cdot \sem{\FF_2}{\sigma}{\interpret}~.
	\]
\end{theorem}
%
\begin{proof}
	We have 
	%
	\begin{align*}
	    &\sem{\FF_1 \cdot \FF_2}{\sigma}{\interpret} \\
	    %
	    \eeq & \sem{\Sup \VVcutnum{1} \colon \Sup \VVcutnum{2} \colon
	    	\VVcutnum{1} \cdot \VVcutnum{2} \cdot \dexp{\FF_1} \cdot \dexp{\FF_2}}{\sigma}{\interpret}
	    \tag{by Definition~\ref{def:product_of_exp}} \\
	    %
	    \eeq &  \sup \setcomp{
	      \sup \setcomp{\sem{
	      	\VVcutnum{1} \cdot \VVcutnum{2} \cdot \dexp{\FF_1} \cdot \dexp{\FF_2}
      	}{\sigma}
	      	{\interpret\statesubst{\VVcutnum{1}}{\RR_1}\statesubst{\VVcutnum{2}}{\RR_2}}}
	         {\RR_2 \in \PosRats}    
                      }{\RR_1 \in \PosRats}
	    \tag{by definition} \\
	    %
	    \eeq &
	    	\sup \setcomp{\sem{
	    			\VVcutnum{1} \cdot \VVcutnum{2} \cdot \dexp{\FF_1} \cdot \dexp{\FF_2}
	    		}{\sigma}
	    		{\interpret\statesubst{\VVcutnum{1}}{\RR_1}\statesubst{\VVcutnum{2}}{\RR_2}}}
	    	{\RR_1 \in \PosRats~\text{and}~\RR_2 \in \PosRats}    
	    %
	    \tag{algebra} \\
	    %
	    \eeq &
	    \sup \setcomp{\sem{
	    		\VVcutnum{1} \cdot \VVcutnum{2} 
	    	}{\sigma}
	    	{\interpret\statesubst{\VVcutnum{1}}{\RR_1}\statesubst{\VVcutnum{2}}{\RR_2}}}
	    {\RR_1 \in \dcut{\sem{\FF_1}{\sigma}{\interpret}}~\text{and}~\RR_2 \in \dcut{\sem{\FF_2}{\sigma}{\interpret}}}  
	    %
	    \tag{by Corollary~\ref{cor:prod_of_dedekind}} \\
	    %
	    \eeq  & \sem{\FF_1}{\sigma}{\interpret} \cdot \sem{\FF_2}{\sigma}{\interpret}
	    \tag{by Equation~\ref{eqn:product_by_dedeking_cut}}~.
	\end{align*}
	%
\end{proof}

==> pgcl_wp.tex <==
\section{PGCL and Weakest Preexpectations}
\label{sec:pgcl_wp}
%
Throughout this section, we assume that all terms and boolean expressions do not contain logical variables and that all constants are natural numbers.
%
\subsection{PGCL}

Programs $\cc$ in the \emph{probabilistic guarded command language}, denoted $\pgcl$, adhere to the grammar
%
\begin{align*}
\cc \qqlongrightarrow 	
%
%
&  \qmid \SKIP 	\tag{effectless program} \\
%
& \qmid \ASSIGN{x}{\TT}	\tag{assignment} \\
%
& \qmid \COMPOSE{\cc}{\cc}	\tag{sequential composition} \\
%
& \qmid \PCHOICE{\cc}{p}{\cc}	\tag{probabilistic choice} \\
%
& \qmid  \ITE{\BB}{\cc}{\cc}	\tag{conditional choice} \\
%
& \qmid  \WHILEDO{\BB}{\cc}	\tag{while loop} \\
\end{align*}
%
where
%
\begin{itemize}
	 \item $\TT$ is an arithmetic expression,
	 %
	 \item $p \in [0,1] \cap \PosRats$ is a rational probability, and
	 %
	 \item $\BB$ is a boolean expression (called \emph{guard}).
\end{itemize}
%
We denote by $\Vars(\cc)$ the set of variables occurring in $\cc$. Notice that $\Vars(\cc)$ is finite.
%
\subsection{Weakest Preexpectations}
%
\subsubsection{Expectations}

An expectation $\ff \colon \States \to \PosRealsInf$ is a map from program states to non-negative reals or infinity. We denote the set of all expectations by $\E$. We strictly distinguish between \emph{expectations}, denoted by $\ff$, $\fg$, $\fh$,\ldots, 
which are maps, and \emph{syntactic expectations}, which are syntactical objects.
We define a partial order $\leq$ on expectations pointwise by
%
\[
\ff \lleq \fg \qquad \text{iff} \qquad \forall \sigma  \in \States \colon \ff(\sigma) \lleq \fg(\sigma)~.
\]
%
Arithmetic operations, infima, and suprema of expectations are also understood pointwise. Given an expectation $\ff$, we denote by
%
\[
   \Vars(\ff) \eeq \setcomp{x \in \Vars}{\exists \sigma \in \States \colon \exists n,n' \in \Nats  \colon \ff(\sigma\statesubst{x}{n}) \neq \ff(\sigma\statesubst{x}{n'})}
\]
%
the set of variables \enquote{occurring} in $\ff$. Throughout this work, we restrict to expectations $\ff$ with $|\Vars(\ff)| < \infty$.

Given an expectation $\ff$, a program variable $x$, and a term $\TT$, we denote by
%
\[
\ff\subst{x}{\TT} \eeq \lambda \sigma \mydot  \ff(\sigma \statesubst{x}{\sem{\TT}{\sigma}{}})
\]
%
the \enquote{substitution} of $x$ by $\TT$ in $\ff$. Furthermore, we employ the \emph
{iverson bracket} notation \cite{Iverson1962} $\iverson{\BB}$ to cast boolean expressions  without logical variables into expectations, i.e.\
%
\begin{align}
\label{eqn:sem_iverson}
\iverson{\BB} \eeq \lambda \sigma \mydot 
\begin{cases}
1, &\text{if}~\sem{\BB}{\sigma}{} = \true \\
%
0, &\text{if}~ \sem{\BB}{\sigma}{}= \false~.
\end{cases}
\end{align}
%
Whether $\iverson{\BB}$ denotes an expectation or a syntactic expectation will be clear from the context.
%
\subsubsection{The Weakest Preexpectation Calculus}
\input{fig_wp}
The \emph{weakest preexpectation transformer}
%
\[
\wpsymbol \colon \pgcl \to (\E \to \E)
\]
%
is defined according to the rules given in Figure~\ref{table:wp}. We call $\wp{\cc}{\ff}$ the \emph{weakest preexpectation} of program $\cc$ w.r.t.\ postexpectation $\ff$. 

Loops deserve special attention. Given a loop $\WHILEDO{\BB}{\cc'}$ and a postexpectation $\ff$, we call
%
\[
\charwp{\BB}{\cc'}{\ff}\colon \E \to \E, \qquad \fg \mapsto \iverson{\neg \guard} \cdot \ff + \iverson{\BB} \cdot \wp{\cc'}{\fg}
\]
%
the \emph{$\wpsymbol$-characteristic functional} of $\WHILEDO{\BB}{\cc'}$ w.r.t.\ postexpectation $\ff$. We can thus recast the weakest preexpectation of a loop as 
%
\[
\wp{\WHILEDO{\BB}{\cc'}}{\ff}
\eeq
\lfp \fg \mydot \charwp{\BB}{\cc'}{\ff}(\fg)~,~\text{i.e.}
\]
%
$\wp{\WHILEDO{\BB}{\cc'}}{\ff}$ is the \emph{least} (w.r.t.\ to our ordering $\leq$ on expectations)
fixedpoint of $\charwp{\BB}{\cc'}{\ff}$. 
We denote by $\charwpn{\BB}{\cc'}{\ff}{n}(0)$  the $n$-fold application of
$\charwp{\BB}{\cc'}{\ff}$ to its argument, i.e.\
%
\[
\charwpn{\BB}{\cc'}{\ff}{0}(0) \eeq 0
\qquad \text{and} \qquad
\charwpn{\BB}{\cc'}{\ff}{n+1}(0)  \eeq \charwp{\BB}{\cc'}{\ff}(\charwpn{\BB}{\cc'}{\ff}{n}(0) )~.
\]
%
Since $(\E, \leq)$ is a complete lattice and since $\charwp{\BB}{\cc'}{\ff}$ is Scott-continuous~\cite{benni_diss}, the Kleene Fixedpoint Theorem~\cite{abramsky_domain_theory} yields
a characterization of this fixedpoint:
\begin{lemma}
	\label{lem:kleene_for_wp}
	Let $\cc = \WHILEDO{\BB}{\cc'}$ be a loop and let $\ff$ be an expectation. We have
	%
	\[
	\wp{\WHILEDO{\BB}{\cc'}}{ \ff}
	%
	\eeq
	\lfp \fg \mydot \charwp{\BB}{\cc'}{\ff}(\fg)
	%
	\eeq
	\sup_{n \in \Nats} \charwpn{\BB}{\cc'}{\ff}{n}(0)~,
	\]
\end{lemma}
%


\subsection{A More Operational Denotational View}
%
Given a finite set of program variables $\varseq{x} = \{ x_0,\ldots, x_{n-1}\}$,
 we define an equivalence relation $\equivstatesrel{\varseq{x}}$ on states by
%
\[
  \equivstates{\sigma_1}{\varseq{x}}{\sigma_2}
  \qquad
  \text{iff}
  \qquad 
  \forall x \in \varseq{x}\colon \sigma_1(x) = \sigma_2(x)~.
\]
%
We always assume a fixed set $\partitionedstates{x} \subseteq \States$ that contains \emph{exactly one} state from each equivalence class.
%
Furthermore, given a state $\sigma \in \States$, we define the \emph{characteristic expectation} expectation $\statepred{\sigma}{\varseq{x}}$ of $\sigma$ (w.r.t.\ $\varseq{x}$) as
%
\[
 \statepred{\sigma}{\varseq{x}} \ddefeq \iverson{x_0 = \sigma(x_0) \wedge \ldots \wedge x_n = \sigma(x_{n-1})}~.
\]
%
The expectation $\statepred{\sigma}{\varseq{x}}$ evaluates to $1$ on state $\sigma'$ if $\sigma$ and $\sigma'$ coincide on all $x \in \varseq{x}$, and to $0$ otherwise. If clear from the context, we often omit the subscribt $\varseq{x}$ and simply write $\statepred{\sigma}{}$. Notice that if $\Vars(\ff) \subseteq \varseq{x}$ for some expectation $\ff$, then $\equivstates{\sigma_1}{\varseq{x}}{\sigma_2}$
implies $\ff(\sigma_1) = \ff(\sigma_2)$.
%
\begin{theorem}
	\label{thm:wp_prob_times_exp}
	Let $\cc$ be a program and $\ff$ be an expectation. Furthermore, let $\varseq{x}$ be a finite set of program variables with $\Vars(c) \cup \Vars(\ff) \subseteq \varseq{x}$. We have
	%
	\[
	   \wp{\cc}{\ff} \eeq \lambda \sigma_0 \mydot \sum_{\sigma \in \partitionedstates{x}} 
	      \wp{\cc}{\statepred{\sigma}{}}(\sigma_0) \cdot \ff(\sigma)~. 
	\]
\end{theorem}
%
\begin{proof}
	By induction on the structure of $\cc$. See Appendix~\ref{proof:wp_prob_times_exp}.
\end{proof}
%
%
As usual, the empty product equals $1$.
%
 \begin{theorem}
   \label{thm:wp_loop_as_sum}
	 Let $\cc = \WHILEDO{\BB}{\cc'}$ be a loop and $\ff$ be an expectation. Furthermore, let $\varseq{x}$ be a finite set of program variables with $\Vars(c) \cup \Vars(\ff) \subseteq \varseq{x}$.  For every $k \in \Nats$, we have
	%
	\begin{align*}
	    &\charwpn{\BB}{\cc'}{\ff}{k}(0)  \\
	    %
	    \eeq &\lambda \sigma_0 \mydot
	    \sum_{\sigma_0,\ldots,\sigma_{k-1} \in \partitionedstates{x}}
	    (\iverson{\neg \BB} \cdot \ff)(\sigma_{k-1})
	    \cdot
	    \prod\limits_{i=0}^{k-2} \wp{\ITE{\BB}{\cc'}{\SKIP}}{\statepred{\sigma_{i+1}}{}}(\sigma_i)~.
	\end{align*}
	%
	Furthermore, it holds that
	%
	\begin{align*}
	&\wp{\WHILEDO{\BB}{\cc'}}{\ff}  \\
	%
	\eeq &\lambda \sigma_0 \mydot \sup_{k \in \Nats}
	\sum_{\sigma_0,\ldots,\sigma_{k-1} \in \partitionedstates{x}}
	(\iverson{\neg \BB} \cdot \ff)(\sigma_{k-1})
	\cdot
	\prod\limits_{i=0}^{k-2} \wp{\ITE{\BB}{\cc'}{\SKIP}}{\statepred{\sigma_{i+1}{}}{}}(\sigma_i)~.
	\end{align*}
	%
\end{theorem}
%
\begin{proof}
	This is a consequence of Lemma~\ref{lem:kleene_for_wp} and Theorem~\ref{thm:wp_prob_times_exp}. See the case $\cc = \WHILEDO{\BB}{\cc_1}$
	in the proof~\ref{proof:wp_prob_times_exp} of Theorem~\ref{thm:wp_prob_times_exp}.
\end{proof}
%
%
\subsection{Encoding (Sequences of) Program States}
Fix a finite set $\varseq{x} = \{x_0,\ldots,x_{k-1}\}$ of program variables.
Every $\gnum$ satisfying $\sequence{\gnum}{k}$ encodes \emph{exactly one}
$\sigma \in \partitionedstates{x}$. Given such a $\sigma \in \partitionedstates{x}$, the unique G\"odel number encoding $\sigma$, which we denote by $\seqnum{\sigma}_{\varseq{x}}$, is the number satisfying
%
\[
 \sequence{\seqnum{\sigma}_{\varseq{x}}}{k} ~{}\wedge{}~\bigwedge\limits_{i=0}^{k-1}
     \seqelem{\seqnum{\sigma}_{\varseq{x}}}{i}{\sigma(x_i)}~.
\]
%
%
The fact that $\gnum$ is the G\"odel number of the \emph{current} state $\sigma$ is expressed by
%
\[
   \encodesstate{x}{\gnum} \ddefeq \sequence{num}{k} ~{}\wedge{}~\bigwedge\limits_{i=0}^{k-1}
   \seqelem{\gnum}{i}{x_i}~.
\]



Now let $\sigma_0,\ldots,\sigma_{n-1} \in \partitionedstates{x}$ be a sequence of states of length $n$. The unique G\"odel number encoding $\sigma_0,\ldots,\sigma_{n-1} $, which we denote by $\stateseqnum{\sigma_0,\ldots,\sigma_{n-1}}_{\varseq{x}}$, is the number satisfying
%
\[
  \sequence{\stateseqnum{\sigma_0,\ldots,\sigma_{n-1}}_{\varseq{x}}}{n} ~{}\wedge{}~\bigwedge\limits_{i=0}^{n-1}
  \seqelem{\stateseqnum{\sigma_0,\ldots,\sigma_{n-1}}_{\varseq{x}}}{i}{\seqnum{\sigma_i}_{\varseq{x}}}~.
\]
%
Given an interpretation $\interpret$,
the fact that some $\gnum$ is the G\"odel number of some sequence $\sigma_0,\ldots,\sigma_{\interpret(\VV-1)} \in \partitionedstates{x}$ of states of length $\interpret{\VV}$ with $\sigma_0$ being the \emph{current} program state is expressed by the formula
%
\begin{align*}
%
     &\stateseq{x}{\gnum}{\VV}  \\
     %
     \ddefeq& \sequence{\gnum}{\VV} \wedge \left( \exists \VV' \colon \seqelem{\gnum}{0}{\VV'} \wedge \encodesstate{x}{\VV'} \right) \\
     %
     &\wedge \forall \VU \colon \forall \VV' \colon \left( ( \VU <\VV \wedge\seqelem{\gnum}{\VU}{\VV'} )\longrightarrow \sequence{\VV'}{k} \right)~.
     %
\end{align*}
%
Notice that for every sequence $\sigma_0,\ldots,\sigma_{n-1}$ of states of length $n$ there is \emph{exactly one} $\gnum$ satisfying $\stateseq{x}{\gnum}{n}$.
If clear from the context, we often omit the subscript $\varseq{x}$ and simply write $\seqnum{\sigma}$ (resp.\ $\stateseqnum{\sigma_0,\ldots,\sigma_{n-1}}$) instead of $\seqnum{\sigma}_{\varseq{x}}$ (resp.\ $\stateseqnum{\sigma_0,\ldots,\sigma_{n-1}}_{\varseq{x}}$).

==> prenex.tex <==
% !TEX root = ./main.tex

\section{Normal Forms}
\label{sec:normalforms}

\subsection{Prenex Normal Form}
We attempt to bring expectations into prenex normal form, i.e., we want to rewrite any expectation~$\FF$ into a \emph{semantically equivalent} expectation of the form
%
\begin{align*}
	\Quant_1 \VV_1 \ldots \Quant_k \VV_k  \colon \FF'~,
\end{align*}
%
where $\Quant_i \in \{\Sup, \Inf\}$ and $\FF'$ is \enquote{quantifier}--free, i.e.\ contains neither \Sup{} nor \Inf.

The following lemma justifies that any expectation can be transformed into an equivalent one in prenex normal form by iteratively pulling out quantifiers.
In case the quantified logical variable already appears in the expectation the quantifier is pulled over, we rename it by a fresh one first.


\begin{lemma}[Prenex Transformation Rules]
\label{thm:prenex-rules}
 For all expectations \FF, $\FF_1$, $\FF_2$, terms $\TT$, and Boolean expressions $\BB$, quantifiers $\Quant \in \{\Sup, \Inf\}$, and fresh logical variables $\VV'$, the following equivalences hold:
%
\begin{enumerate}
  %
  \item\label{thm:prenex-rules:plus-left} 
  $(\Quant \VV\colon \FF_1) \pplus \FF_2 \qquad\equiv\qquad \Quant \VV'\colon \FF_1\subst{\VV}{\VV'} \pplus \FF_2$, 
  %
  \item\label{thm:prenex-rules:plus-right} 
  $\FF_1 \pplus (\Quant \VV'\colon \FF_2) \qquad\equiv\qquad \Quant \VV'\colon \FF_1 \pplus \FF_2\subst{\VV}{\VV'}$,
  %
  \item\label{thm:prenex-rules:mult-term} 
  $\TT \ccdot \Quant \VV\colon \FF \qquad\equiv\qquad \Quant \VV'\colon \TT \cdot \FF\subst{\VV}{\VV'}$, \qquad and
  %
  \item\label{thm:prenex-rules:mult-guard} 
  $\iverson{\BB} \ccdot \Quant \VV\colon \FF \qquad\equiv\qquad \Quant \VV'\colon \iverson{\BB} \cdot \FF\subst{\VV}{\VV'}$.
  %
\end{enumerate}
%
\end{lemma}

In order to prove the above lemma, we rely on a few standard properties of infima and suprema over sets of real numbers which are collected below.

\begin{lemma}[folklore/find good reference]
\label{thm:prenex:aux}
Let $c \in \PosReals$ and $A,B \subseteq \PosRealsInf$. Then, we have:
\begin{enumerate}
%
\item\label{thm:prenex:aux:sup-mult}
        $c \cdot \sup A \qqeq \sup \{ c \cdot a \mmid a \in A \}$,
%
\item\label{thm:prenex:aux:inf-mult}
$c \cdot \inf A \qqeq \inf \{ c \cdot a \mmid a \in A \}$,
%
\item\label{thm:prenex:aux:sup-plus}
$(\sup A) + (\sup B) \qqeq \sup \{ a + b \mmid a \in A, b \in B \}$, and
%
\item\label{thm:prenex:aux:inf-plus}
$(\inf A) + (\inf B) \qqeq \inf \{ a + b \mmid a \in A, b \in B \}$,
%
\item\label{thm:prenex:aux:singleton}
if $A$ is a singleton, i.e.,  $A = \{ a \}$, then $\sup A = \inf A = a$,
%
\end{enumerate}
where we interpret $0 \cdot \infty = 0$.
\cmcommentinline{I'm sure we can find this in a textbook for $A,B \subseteq \PosReals$. Perhaps we have to prove it for $A,B \subseteq \PosRealsInf$ ourselves. Still, this is easier on this level considering expectations and proceeding by case distinction to deal with $\infty$.}
\end{lemma}

\begin{proof}[Proof of~Lemma~\ref{thm:prenex-rules}]
%
By definition of equivalence between expectations, we have 
\begin{align*}
    \FF_1 \equiv \FF_2 
    \qiff 
    \forall \sigma \forall \interpret\colon \sem{\FF_1}{\sigma}{\interpret} \eeq \sem{\FF_2}{\sigma}{\interpret}.
\end{align*}
Let us thus fix an arbitrary state $\sigma$ and an arbitrary interpretation $\interpret$, respectively.

To prove Lemma~\ref{thm:prenex-rules}~(\ref{thm:prenex-rules:plus-left}) for $\Quant = \Sup$, we proceed as follows:
%
\begin{align*}
%
& \sem{(\SupV{\VV} \FF_1) \pplus \FF_2}{\sigma}{\interpret} \\
%
\eeq & 
\sup~\setcomp{\sem{\FF_1}{\pstate}{\interpret\statesubst{\VV}{\RR}}}{\RR \in \PosRats} 
\pplus \sem{\FF_2}{\pstate}{\interpret} 
\tag{Semantics of expecations} \\
%
\eeq & 
\sup~\setcomp{\sem{\FF_1}{\pstate}{\interpret\statesubst{\VV}{\RR}}}{\RR \in \PosRats} 
\pplus 
\sup~\left\{\sem{\FF_2}{\pstate}{\interpret}\right\}
\tag{Lemma~\ref{thm:prenex:aux}~(\ref{thm:prenex:aux:singleton})} \\
%
\eeq & 
\sup~\setcomp{\sem{\FF_1\subst{\VV}{\VV'}}{\pstate}{\interpret\statesubst{\VV'}{\RR}} + \sem{\FF_2}{\pstate}{\interpret\statesubst{\VV'}{\RR}}}{\RR \in \PosRats} 
\tag{Lemma~\ref{thm:prenex:aux}~(\ref{thm:prenex:aux:sup-plus}), $\VV'$ fresh} \\
%
\eeq & 
\sem{\SupV{\VV'} \FF_1\subst{\VV}{\VV'} \pplus \FF_2 }{\sigma}{\interpret}.
\tag{Semantics of expecations}
\end{align*}
%
The proofs for $\Quant = \Inf$ as well as the proof of Lemma~\ref{thm:prenex-rules}~(\ref{thm:prenex-rules:plus-right}) are completely analogous.
%

%
To prove Lemma~\ref{thm:prenex-rules}~(\ref{thm:prenex-rules:mult-term}) for $\Quant = \Inf$, we proceed as follows:
\begin{align*}
%
& \sem{\TT \cdot \InfV{\VV} \FF}{\sigma}{\interpret} \\
%
\eeq & 
\sem{\TT}{\sigma}{\interpret} \cdot \inf \setcomp{ \sem{\FF}{\sigma}{\interpret\statesubst{\VV}{\RR}} }{ \RR \in \PosRats }
\tag{Semantics of expectations} \\
%
\eeq & 
\inf \setcomp{\sem{\TT}{\sigma}{\interpret} \cdot \sem{\FF}{\sigma}{\interpret\statesubst{\VV}{\RR}} }{ \RR \in \PosRats }
\tag{Lemma~\ref{thm:prenex:aux}~(\ref{thm:prenex:aux:inf-mult})} \\
%
\eeq & 
\inf \setcomp{\sem{\TT}{\sigma}{\interpret\statesubst{\VV'}{\RR}} \cdot \sem{\FF\subst{\VV}{\VV'}}{\sigma}{\interpret\statesubst{\VV'}{\RR}} }{ \RR \in \PosRats }
\tag{$\VV'$ fresh} \\
%
\eeq & 
\sem{\InfV{\VV'} \TT \cdot \FF\subst{\VV}{\VV'}}{\sigma}{\interpret} 
\tag{Semantics of expectations}.
%
\end{align*}
%
The proofs for $\Quant = \Sup$ as well as the proof of Lemma~\ref{thm:prenex-rules}~(\ref{thm:prenex-rules:mult-guard}) are completely analogous.
%
\end{proof}

%Terms and Iverson brackets are by definition quantifier--free, thus trivially in prenex normal form.
%For addition and multiplication, the rules are provided in \autoref{tab:pnf}. 
%%
%%
%%\begin{table}[b]
%%	\caption{Rules for transforming composite expectations into prenex normal form.}
%%	\label{tab:pnf}
%%	\renewcommand{\arraystretch}{1.5}
%%	\begin{tabular}{l@{\qquad}l@{\qquad}l@{\qquad}l}	
%%		\textbf{Expectation $\boldsymbol{h}$} & $\boldsymbol{\boldsfsymbol{Prenex}(h)}$ & \textbf{Side conditions} & \\
%%		\hline\hline
%%		%
%%		%
%%		$(\Quant v\colon f) \pplus g$ & $\Quant u: f\subst{v}{u} + g$ & $u$ is fresh & \gray{(add-l)} \\
%%		%
%%		$f \pplus (\Quant v\colon g)$ & $\Quant u: f + g\subst{v}{u}$ & $u$ is fresh & \gray{(add-r)} \\[.5em]
%%		%
%%		\hline\\[-1.5em]
%%		%
%%		$(\Quant v\colon f) \ccdot g$ & $\Quant v\colon f \cdot g$ & $g$ is quantifier-free & \gray{(mult-l)} \\
%%		%
%%		$f \ccdot (\Quant v\colon g)$ & $\Quant v\colon f \cdot g$ & $f$ is quantifier-free & \gray{(mult-l)} \\[.5em]
%%		%
%%		$(\Sup v\colon f) \ccdot (\Sup w\colon g)$ & $\Sup u \: \Sup z\colon f\subst{v}{u} \cdot g\subst{w}{z}$ & $u$ and $z$ are fresh & \gray{(mult-ss)} \\
%%		%
%%		$(\Inf v\colon f) \ccdot (\Inf w\colon g)$ & $\Inf u \: \Inf z\colon f\subst{v}{u} \cdot g\subst{w}{z}$ & $u$ and $z$ are fresh & \gray{(mult-ii)} \\
%%		%
%%		$(\blue{\Sup v\colon f}) \ccdot (\orange{\Inf w\colon g})$ & $\blue{\Sup u} \: \orange{\Inf z}\colon \blue{f\subst{v}{u}} \cdot \orange{g\subst{w}{z}}$ & $u$ and $z$ are fresh & \gray{(mult-si)} \\
%%		%
%%		$(\orange{\Inf v\colon f}) \ccdot (\blue{\Sup w\colon g})$ & $\blue{\Sup z} \: \orange{\Inf u}\colon \orange{f\subst{v}{u} }\cdot \blue{g\subst{w}{z}}$ & $u$ and $z$ are fresh & \gray{(mult-is)} \\[.5em]
%%		\hline\\[-1.5em]
%%		\multicolumn{4}{c}{$u$ and $z$ being \emph{fresh} means that $u$ and $z$ are freshly drawn logical}\\[-.6125em]
%%		\multicolumn{4}{c}{variables from $\LVars$ that occur neither in $f$ nor in $g$.}\\
%%	\end{tabular}
%%	\renewcommand{\arraystretch}{1}
%%\end{table}%
%%
%%
%For addition (rules (add-l) and (add-r)), we can just pull quantifiers one after the other out of the summands in front of the sum.
%We merely have to rename the bound variable such that the quantified variable name does not occur in the other summand.
%We can do the same for multiplication, if we pull out quantifiers from one factor when the \emph{other} factor is quantifier--free (rules (mult-l) and (mult-r)).
%If, for multiplication, both factors contain quantifiers, we can pull out the leading two quantifiers at the same time, again subject to appropriate renaming (rules (mult-ss) and (mult-ii)).
%
%The situation is more subtle when facing a multiplication with a leading $\Sup$ in one factor and a leading $\Inf$ in the other factor. 
%In this case, we always have to pull out the $\Sup$--quantifier first and then the $\Inf$--quantifier.
%Intuitively, the reason is that $0 \cdot \infty = 0$.
%ADD MORE EXPLANATION HERE.


\subsection{Summation Normal Form}

\begin{lemma}
	\label{lem:quantifier_free_smf}
	Let $\FF \in \SyntE$ be quantifier-free. Then there is an $n \in \Nats$, boolean expressions $\BB_1,\ldots,\BB_n$, and terms $\TT_1,\ldots,\TT_n$ such that $\FF$ is equivalent to an expectation $\FF'$ given by
	%
	\[
		\FF' \eeq \sum\limits_{i=1}^{n} \iverson{\BB_i}\cdot \TT_i ~,
	\]
	%
	where the above sum is a shorthand for $\iverson{\BB_1}\cdot \TT_1 + \ldots + \iverson{\BB_n}\cdot \TT_n$.
\end{lemma}
%
%
%
%
\begin{theorem}[Summation Normal Form]
	Every syntactic expectation $\FF$ is equivalent to an expectation $\FF'$ in \emph{summation normal form}, i.e.\
	$\FF'$ is of the form
	%
	\[
		\FF' \eeq \Quant_1 \VV_1 \ldots \Quant_k \VV_k \colon \sum\limits_{i=1}^{n} \iverson{\BB_i}\cdot \TT_i ~.
	\]
\end{theorem}
%
\begin{proof}
	Assume w.l.o.g.\ that $\FF$ is in prenex normal form (Lemma~\ref{thm:prenex-rules}), i.e.\ $\FF$ is of the form
	%
	\[
		\FF \eeq \Quant_1 \VV_1 \ldots \Quant_k \VV_k \colon \FF'~,
	\]
	%
	where $\FF'$ is quantifier-free. Now, by Lemma~\ref{lem:quantifier_free_smf}, $\FF'$ is equivalent to an expectation of the form
	%
	\[
		\sum\limits_{i=1}^{n} \iverson{\BB_i}\cdot \TT_i~,
	\]
	%
	which completes the proof.
\end{proof}
%
%
\subsection{Dedekind Normal Form}
%
This section presents a \emph{Dedekind normal form} of syntactic expectations. The Dedekind normal form is motivated by the notion of \emph{Dedekind cuts} [CITATION MISSING].
A Dedekind cut $\dcut{a} \subseteq \Reals$ of a real number $a \in \Reals$ is the set of all rationals strictly smaller than $a$, i.e.\
%
\[
	\dcut{a} \eeq \setcomp{r \in \Rats}{r < a}~.
\]
%
An important property that we will make heavy use of is that every real number $a$ is obtained from taking the supremum of the corresponding Dedekind cut $\dcut{a}$, i.e.\
\[
	a \eeq \sup \dcut{a}~.
\]
%
In the realm of \emph{all} reals, it is required that a Dedekind cut is neither equal to the empty set nor the whole set of rationals $\Rats$. Since we, however, operate in the realm of non-negative reals with infinity $\PosRealsInf$, we \emph{do} allow for empty cuts or for cuts equal to $\PosRats$. More formally, we define:
%
\begin{definition}[Dedekind Cuts of Non-Negative Reals]
	The \emph{Dedekind cut} $\dcut{a}$ of some $a \in \PosRealsInf$ is defined as
	%
	\[
		\dcut{a} \eeq \setcomp{r \in \PosRats}{ r < a}~.
	\]
\end{definition}
%
\noindent
Notice that the Dedekind cut $D_0$ (resp.\ $D_\infty$) of $0$ (resp.\ $\infty$) is the empty set (resp.\ $\PosRats$). Since the supremum of $\emptyset$ (resp.\ $\PosRats$) over $\PosRealsInf$ is $0$ (resp.\ $\infty$), our definition preserves the property that $a \eeq \sup \dcut{a}$ for every $a \in \PosRealsInf$.

\begin{theorem}
	\label{thm:dedekind_nf}
	Let 
	%
	\[
		\FF \eeq \Quant_1 \VV_1 \ldots \Quant_k \VV_k \colon \sum\limits_{i=1}^{n} \iverson{\BB_i}\cdot \TT_i
	\]
	%
	be a syntactic expectation in summation normal form, and let $\VVcut$ be a fresh logical variable.
	Define the \emph{Dedekind normal form} $\dexp{\FF}$ of $\FF$ by
	%
	\[
		\dexp{\FF} \eeq \Quant_1 \VV_1 \ldots \Quant_k \VV_k \colon
		\iverson{\bigwedge_{((B_1, T_1), \ldots, (B_n, T_n)) \in \bigtimes_{i = 1}^{n} \{ (b_i, t_i), (\neg b_i, 0) \}}
		\bigwedge_{i=1}^{n} B_i \implies \VVcut < \sum_{i=0}^{n} T_i }~.
	\]
	Then for all programm states $\sigma$ and all interpretations $\interpret$, we have
	%
	\[
			\sem{\dexp{F}}{\sigma}{\interpret} 
			\eeq
			\begin{cases}
			   1, & \text{if}~\interpret(\VVcut) < \sem{f}{\sigma}{\interpret} \\
			   %
			   0, &\text{otherwise}~.
			\end{cases}
	\]
\end{theorem}
%
\begin{proof}
	First notice that indeed $\sem{\dexp{f}}{\sigma}{\interpret} \in \{0,1\}$. We proceed by induction on $k$. \\ \\
	%
	\noindent
	\emph{Base case $k=0$.} In this case,
	%
	\[
		\FF \eeq \sum\limits_{i=1}^{n} \iverson{\BB_i}\cdot \TT_i~.
	\]
	%
	Now there is \emph{exactly one} $((B_1', T_1'), \ldots, (B_n', T_n')) \in \bigtimes_{i = 1}^{n} \{ (b_i, t_i), (\neg b_i, 0) \}$ such that
	\[
	 \sem{\bigwedge_{i=1}^{n} B_i'}{\sigma}{\interpret} \eeq \true~.
	\]
	%
	Hence, we have
	%
	\begin{align*}
		& \sem{f}{\sigma}{\interpret} \\
		%
		\eeq & \sem{\sum\limits_{i=1}^{n} \iverson{\BB_i}\cdot \TT_i}{\sigma}{\interpret}
		\tag{by definition} \\
		%
		\eeq & \sem{\sum\limits_{i=1}^{n} T_i'}{\sigma}{\interpret}~.
		\tag{since $\sem{\iverson{b_j}}{\sigma}{\interpret}$ = 0 if $B_j = \neg b_j$}
	\end{align*}
	%
	This is gives us
	%
	\begin{align*}
	    	&\sem{\dexp{F}}{\sigma}{\interpret}  \eeq 1 \\
	    	%
	    	\text{iff} \quad & \sem{\iverson{\bigwedge_{((B_1, T_1), \ldots, (B_n, T_n)) \in \bigtimes_{i = 1}^{n} \{ (b_i, t_i), (\neg b_i, 0) \}}
	    			\bigwedge_{i=1}^{n} B_i \implies \VVcut < \sum_{i=0}^{n} T_i }}{\sigma}{\interpret} \eeq 1 
    			\tag{by definition}\\
    		%
    		\text{iff} \quad & \sem{\iverson{\bigwedge_{i=1}^{n} B_i' \implies \VVcut < \sum_{i=0}^{n} T_i' }}{\sigma}{\interpret} \eeq 1 
    		\tag{by above reasoning}\\
    		%
    		\text{iff} \quad & \sem{\iverson{\VVcut < \sum_{i=0}^{n} T_i' }}{\sigma}{\interpret} \eeq 1 
    		\tag{left-hand side of implication evaluates to $\true$ by construction}\\
    		%
    		\text{iff} \quad & \interpret(\VVcut) \LL \sem{\sum_{i=0}^{n} T_i'}{\sigma}{\interpret} 
    		\tag{by definition}\\
    		%
    		\text{iff} \quad & \interpret(\VVcut) \LL \sem{f}{\sigma}{\interpret}~. 
    		\tag{by above reasoning}\\
	\end{align*}
	%
	As the induction hypothesis now suppose that for some arbitrary, but fixed, $k \in \Nats$, all states$\sigma$, all interpretations $\interpret$, and all syntactic expectations
	%
	\[
		\FF \eeq \Quant_1 \VV_1 \ldots \Quant_k \VV_k \colon \sum\limits_{i=1}^{n} \iverson{\BB_i}\cdot \TT_i
	\]
	%
	it holds that 
	%
	\[
	\sem{\dexp{F}}{\sigma}{\interpret} 
	\eeq
	\begin{cases}
	1, & \text{if}~\interpret(\VVcut) < \sem{f}{\sigma}{\interpret} \\
	%
	0, &\text{otherwise}~.
	\end{cases}
	\]
	%
	%
	\emph{Induction step.} We now consider an expectation of the form
	%
	\[
		\FF \eeq \Quant_1 \VV_1 \ldots \Quant_{k+1} \VV_{k+1} \colon \sum\limits_{i=1}^{n} \iverson{\BB_i}\cdot \TT_i~.
	\]
	%
	Write $\dexp{\FF} = \Quant_1 \VV_1 \ldots \Quant_{k+1} \VV_{k+1} \colon \FF'$.
	We distinguish the cases $\Quant_1 = \Sup$ and $\Quant_1 = \Inf$. \\ \\
	%
	\noindent
	\emph{The case $\Quant_1 = \Sup$.} We have
	%
	\begin{align*}
	     & \sem{\dexp{f}}{\sigma}{\interpret} \eeq  1 \\
	     %
	     \text{iff} \quad & \sem{ \Sup \VV_1 \ldots \Quant_{k+1} \VV_{k+1} \colon \FF'}{\sigma}{\interpret} \eeq  1 
	     \tag{by definition} \\
	     %
	     \text{iff} \quad & \sup 
	     		\setcomp{   \sem{\Quant_2 \VV_2 \ldots \Quant_{k+1} \VV_{k+1} \colon \FF' }{\sigma}{\interpret\statesubst{\VV_1}{\RR}}   }{\RR \in \PosRats} \eeq 1
	     \tag{by definition} \\
	     %
	     \text{iff}\quad & \text{there is}~\RR \in \PosRats~\text{with}~
	     	\sem{\Quant_2 \VV_2 \ldots \Quant_{k+1} \VV_{k+1} \colon \FF'}{\sigma}{\interpret\statesubst{\VV_1}{\RR}} \eeq 1
	     \tag{expression on the left-hand side of the set comprehension evaluates to either $0$ or $1$} \\
	     %
	     \text{iff}\quad & \text{there is}~\RR \in \PosRats~\text{with}~
	     \interpret\statesubst{\VV_1}{\RR}(\VVcut) \LL  \sem{\Quant_2 \VV_2 \ldots \Quant_{k+1} \VV_{k+1} \colon \FF'}{\sigma}{\interpret\statesubst{\VV_1}{\RR}} 
	     \tag{by I.H.} \\
	     %
	     \text{iff}\quad & \text{there is}~\RR \in \PosRats~\text{with}~
	      \interpret(\VVcut) \LL  \sem{\Quant_2 \VV_2 \ldots \Quant_{k+1} \VV_{k+1} \colon \FF'}{\sigma}{\interpret\statesubst{\VV_1}{\RR}} 
	     \tag{$\VV_1 \neq \VVcut$ by construction} \\
	     %
	     \text{iff}\quad & 
	     \interpret(\VVcut) \LL  \sup \setcomp{\sem{\Quant_2 \VV_2 \ldots \Quant_{k+1} \VV_{k+1} \colon \FF'}{\sigma}{\interpret\statesubst{\VV_1}{\RR}} }{\RR \in  \PosRats \}}
	     \tag{see below} \\
	     %
	     \text{iff}\quad & 
	     \interpret(\VVcut) \LL   \sem{\Sup \VV_1 \Quant_2 \VV_2 \ldots \Quant_{k+1} \VV_{k+1} \colon \FF'}{\sigma}{\interpret} 
	     %
	     \tag{by definition}
	\end{align*}
	%
	We justify the second last step as follows. The \enquote{only if}-direction is obvious.
	
	For the \emph{if}-direction, assume for a contradiction that
	%
	\begin{align}
	\label{eq:proof_dedekind_nf_1}
		\interpret(\VVcut) \LL  \sup \setcomp{\sem{\Quant_2 \VV_2 \ldots \Quant_{k+1} \VV_{k+1} \colon \FF'}{\sigma}{\interpret\statesubst{\VV_1}{\RR}} }{\RR \in  \PosRats \}}
	\end{align}
	%
	and
	%
	\begin{align}
	\label{eq:proof_dedekind_nf_2}
		\text{for all}~\RR \in \PosRats~\text{it holds that}~
		\interpret(\VVcut) \ggeq  \sem{\Quant_2 \VV_2 \ldots \Quant_{k+1} \VV_{k+1} \colon \FF'}{\sigma}{\interpret\statesubst{\VV_1}{\RR}} ~.
	\end{align}
	%
	Inequality~\ref{eq:proof_dedekind_nf_2} implies that $\interpret(\VVcut)$ is an upper bound on
	$ \setcomp{\sem{\Quant_2 \VV_2 \ldots \Quant_{k+1} \VV_{k+1} \colon \FF'}{\sigma}{\interpret\statesubst{\VV_1}{\RR}} }{\RR \in  \PosRats \}}$. Hence, $\interpret(\VVcut)$ is greater than or equal to the \emph{least} upper bound of this set. This contradicts Inequality~\ref{eq:proof_dedekind_nf_1}. \\ \\
	%
	%
	\noindent
	\emph{The case $\Quant_1 = \Inf$.} We have
	%
	\begin{align*}
	& \sem{\dexp{f}}{\sigma}{\interpret} \eeq  1 \\
	%
	\text{iff} \quad & \sem{ \Inf  \VV_1 \ldots \Quant_{k+1} \VV_{k+1} \colon \FF'}{\sigma}{\interpret} \eeq  1 
	\tag{by definition} \\
	%
	\text{iff} \quad & \inf 
	\setcomp{   \sem{\Quant_2 \VV_2 \ldots \Quant_{k+1} \VV_{k+1} \colon \FF' }{\sigma}{\interpret\statesubst{\VV_1}{\RR}}   }{\RR \in \PosRats} \eeq 1
	\tag{by definition} \\
	%
	\text{iff}\quad & \text{for all}~\RR \in \PosRats~\text{we have}~
	\sem{\Quant_2 \VV_2 \ldots \Quant_{k+1} \VV_{k+1} \colon \FF'}{\sigma}{\interpret\statesubst{\VV_1}{\RR}} \eeq 1
	\tag{expression on the left-hand side of the set comprehension evaluates to either $0$ or $1$} \\
	%
	\text{iff}\quad & \text{for all}~\RR \in \PosRats~\text{we have}~
	\interpret\statesubst{\VV_1}{\RR}(\VVcut) \LL  \sem{\Quant_2 \VV_2 \ldots \Quant_{k+1} \VV_{k+1} \colon \FF'}{\sigma}{\interpret\statesubst{\VV_1}{\RR}} 
	\tag{by I.H.} \\
	%
	%
	\text{iff}\quad & \text{for all}~\RR \in \PosRats~\text{we have}~
	\interpret(\VVcut) \LL  \sem{\Quant_2 \VV_2 \ldots \Quant_{k+1} \VV_{k+1} \colon \FF'}{\sigma}{\interpret\statesubst{\VV_1}{\RR}} 
	\tag{$\VV_1 \neq \VVcut$ by construction} \\
	%
	\text{iff}\quad & 
	\interpret(\VVcut) \LL  \inf \setcomp{\sem{\Quant_2 \VV_2 \ldots \Quant_{k+1} \VV_{k+1} \colon \FF'}{\sigma}{\interpret\statesubst{\VV_1}{\RR}} }{\RR \in  \PosRats \}}
	\tag{see below} \\
	%
	\text{iff}\quad & 
	\interpret(\VVcut) \LL   \sem{\Inf \VV_1 \Quant_2 \VV_2 \ldots \Quant_{k+1} \VV_{k+1} \colon \FF'}{\sigma}{\interpret} 
	%
	\tag{by definition}
	\end{align*}
	%
	We justify the second last step as follows. The \enquote{if}-direction is obvious.
	
	For the \enquote{only-if}-direction, assume the contrary, i.e.\ assume for a contradiction that
	%
	\begin{align}
	\label{eq:proof_dedekind_nf_3}
		\interpret(\VVcut) \LL  \inf \setcomp{\sem{\Quant_2 \VV_2 \ldots \Quant_{k+1} \VV_{k+1} \colon \FF'}{\sigma}{\interpret\statesubst{\VV_1}{\RR}} }{\RR \in  \PosRats \}}
	\end{align}
	%
	but
	%
	\begin{align}
	\label{eq:proof_dedekind_nf_4}
	%
	\text{there exists}~\RR \in \PosRats~\text{with}~
	\interpret(\VVcut) \ggeq  \sem{\Quant_2 \VV_2 \ldots \Quant_{k+1} \VV_{k+1} \colon \FF'}{\sigma}{\interpret\statesubst{\VV_1}{\RR}}~.
	\end{align}
	%
	Inequality~\ref{eq:proof_dedekind_nf_3} implies that $\interpret(\VVcut)$ is a strict lower bound on $\setcomp{\sem{\Quant_2 \VV_2 \ldots \Quant_{k+1} \VV_{k+1} \colon \FF'}{\sigma}{\interpret\statesubst{\VV_1}{\RR}} }{\RR \in  \PosRats \}}$, which contradicts Inequality~\ref{eq:proof_dedekind_nf_4}. This completes the proof.
\end{proof}

